Existence of singularities in two-Kerr black holes

We show that the angular momentum - area inequality 8\pi |J| =< A for weakly stable minimal surfaces would apply to (I^+)-regular many-Kerr solutions, if any existed. Hence we remove the undesirable hypothesis in the Hennig-Neugebauer proof of non-existence of well behaved two-component solutions.

==> LeeNewcommand.tex <==
%
% run3
%

\newcommand\mcMloc{{\mcM_{\rm loc}}}
\newcommand\rhoS{{\rho_S}}
\newcommand\zS{{z_S}}
\newcommand\zetaS{{\zeta_S}}
\newcommand\ringX{{\mathring{X}}}

\newcommand{\ptccheck}[1]{\mnote{ptcchecked:#1}}
\renewcommand{\ptccheck}[1]{\mnote{\checkmark (ptc #1)}}
\newcommand{\jccheck}[1]{\mnote{jcchecked:#1}}

%% topoorig %%
\newcommand{\docl}{\langle\langle\mcMext^\lambda\rangle\rangle}%
%\newcommand{\mcMext}{\Mext}%
\newcommand{\Mextl}{\Mext^\lambda}%
\newcommand{\Mextls}{\Mext^{\lambda_*}}%
\newcommand{\docls}{\langle\langle \mcMext^{\lambda_*}\rangle\rangle}%
\newcommand{\doclo}{\langle\langle \mcMext^{\lambda_1}\rangle\rangle}%
\newcommand{\doclt}{\langle\langle \mcMext^{\lambda_2}\rangle\rangle}%

%% NormTwistEquations %%

%Krakow
\newcommand{\ub}[1]{\underbrace{#1}}
\newcommand{\dd}[2]{\frac{d #1}{d #2}}
\newcommand{\twogL}{\stackrel{\tiny (2)}{g}}


\newcommand{\hlambda}{\hat \lambda}
\newcommand{\zSigma}{{\mathring{\Sigma}}}
\newcommand{\homega}{\hat \omega}%
%\newcommand{\eN}{=\!\!\big|{_\mcN}}
\newcommand{\eN}{=\!\! {_\mcN}}
\newcommand{\XtoK}{X}

\newcommand{\KtoX}{X}

\newcommand{\Nnmo}{N^{n-1}}

\newcommand{\lnote}[1]{{\bf #1}}


%\newcommand{\olstop}[3]{}%%
%\newcommand{\lstop}[3]{}%%

\newcommand{\lstop}[3]{\noindent=============== End of Lecture #1 on #2 ================%
\\ {\bf{#3}} \ptc{#2}%
\\==============================================%
\vfill\eject}

\newcommand{\olstop}[3]{\ptc{End of Lecture #1 on #2:  #3}}



%% Cortier %%
\newcommand{\mychithree}{\tilde\chi }
\newcommand{\mydotz}[1]{\frac{d #1}{dz}}%
\newcommand{\mychione}{\chi }
\newcommand{\bmydot}[2]{\left(\frac{d#1}{ds}\right)#2}%
\newcommand{\mydot}[1]{\frac{d#1}{ds}}%
\newcommand{\mychitwo}{\mathring \chi }
\newcommand{\myrho}{\theta}
\newcommand{\dmyrho}{\dot\theta}
\newcommand{\mhatg}{g}
\newcommand{\obstruction}{--compatibility}%
\newcommand{\tmcM}{\,\,\,\,\widetilde{\!\!\!\!\mcM}}%
\newcommand{\mutheta}{\theta}
\newcommand{\myb}{b}%
\newcommand{\myc}{\xi_0}%
\newcommand{\myalph}{a}
\newcommand{\mygamma}{\sigma}

%% main0 %%
\newcommand{\xmcop}{X_{\mcO_p}}\newcommand{\xmcopi}{X_{\mcO_{p_i}}}\newcommand{\xmcoq}{X_{\mcO_q}}

%% blackholes %%
\newcommand{\tilr}{\tilde r}%

%% Reall %%
\newcommand{\oldxithree}{\xi_2{}}%
\newcommand{\oldxifour}{\xi_3{}}%
\newcommand{\oldxitwo}{\xi_1{}}%
\newcommand{\xitwo}{\oldxithree}%
\newcommand{\xione}{\oldxitwo}%
\newcommand{\xithree}{\oldxifour}%

%% Characteristic %%
\newcommand{\msqh}{\sqrt{\det h_{EF}}}%
\newcommand{\mysign }{\varepsilon}%
\newcommand{\btheta }{\bar \theta}%
\newcommand{\mysqh}{\sqrt{\det{h_{EF}}}}%%
\newcommand{\myhsqh}{\sqrt{\det{\hat h_{EF}}}}%
\newcommand{\hE}{\hat E}%
\newcommand{\genK}{L}%
\newcommand{\prd}{\frac 1 {\msqh} \partial_r \Big(\msqh\Big)}%
\newcommand{\genL}{\underbar{{\mbox{\emph L}}}\,}%


%% Costa %%
\newcommand{\calSJr}{{\mycal  S}_{(J_0,\rho_0)}}
\newcommand{\Ima}{\mbox{\rm Im}}
\newcommand{\Ker}{{\mathrm{Ker}}}
\newcommand{\sgstatic}{{strictly globally static{}}}
\newcommand{\gstatic}{{globally static{}}}
\newcommand{\riemg}{g}
\newcommand{\riemgz}{g_0}
\newcommand{\hhat}{\ghat}
\newcommand{\DeltaL}{\Delta_{\mathrm L}}
\newcommand{\ghat}{\gamma}%{{\widehat \riemg}}
\newcommand{\hzhat}{\gamma_0}%{{\widehat \riemgz}}
\newcommand{\holder}{H\"older }

\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbZ}{\mathbb{Z}}
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbH}{\mathbb{H}}

\newcommand{\scro}{{\mycal O}}
\newcommand{\Doc}{\doc}%{{\mycal Doc}}
% \newcommand{\scrip}{\scri^{+}}%
% \newcommand{\scrp}{{\mycal I}^{+}}%
% \newcommand{\Scri}{\scri}
\newcommand{\scra}{{\mycal A}}
\newcommand{\Scra}{\cup_{i}\scra_i}
\newcommand{\scru}{{\mycal U}}
\newcommand{\scrw}{{\mycal W}}
\newcommand{\scrv}{{\mycal V}}
\newcommand{\scrs}{{\mycal S}}
\newcommand{\rot}{{\mycal R}}
\newcommand{\khor}{{\mycal H}}

\newcommand{\jlcax}[1]{}
\newcommand{\hahyp}{\,\,\widehat{\!\!\hyp}}%
\newcommand{\mcMext}{\Mext}
\newcommand{\kl}[1]{{(#1)}}
\newcommand{\Kz}{K_\kl 0}
\newcommand{\nic}{}
\newcommand{\mcHp}{{\mcH^+}}
\newcommand{\Sz}{S_0}
\newcommand{\Sone}{\Sz}
\newcommand{\Sonep}{\Sz}%{S_{0,p}}
\newcommand{\Soneq}{S_{0,q}}
\newcommand{\ue}{u_{\epsilon}}
\newcommand{\uee}{u_{\epsilon,\eta}}

%\newcommand{\bmcM}{\,\,\,\,\widetilde{\!\!\!\!\mcM}}
\newcommand{\bfourg}{\widetilde{\fourg}}

\newcommand{\eean}{\nonumber\end{eqnarray}}

\newcommand{\lp}{\ell}

\newcommand{\tSp}{\tilde S_p}
\newcommand{\Sp}{S_p}

\newcommand{\dgtcp}{\dgt}%{(\dgt\cup \zh)}
\newcommand{\dgtc}{\dgt}%{\dgt\cup \zh}

%\newcommand{\id}{{\rm id}}

\newcommand{\hSzR}{\hat S_{0,R}}
\newcommand{\hSts}{\hat S_{\tau,\sigma}}

%\newcommand{\Sone}{\Sz}
%\newcommand{\Sonep}{\Sz}%{S_{0,p}}
%\newcommand{\Soneq}{S_{0,q}}
\newcommand{\Stp}{S_{t,p}}
\newcommand{\Stq}{S_{t,q}}
%\newcommand{\Sz}{S_0}

\newcommand{\bw}{\bar w}
\newcommand{\bzeta}{\bar \zeta}

\newcommand{\zMtwo}{\mathring{M}{}^2}
\newcommand{\Mtwo}{{M}{}^2}
\newcommand{\bMtwo}{{\bar M}{}^2}
\newcommand{\hMtwo}{{\hat M}{}^2}

%\newcommand{\hypext}{\hyp_{\mbox{\scriptsize \rm ext}}}
%\newcommand{\Mtext}{\Sext}%{M_{\mbox{\scriptsize \rm ext}}}
\newcommand{\Mint}{\mcM_{\mbox{\scriptsize \rm int}}}
%\newcommand{\mcMext}{\Mext}

\newcommand{\mcHN}{\mcN}
\newcommand{\mcNH}{\mcH}

%\newcommand{\hS }{{\hat S }}
\newcommand{\hSq}{{\hat S_q}}
\newcommand{\hSp}{{\hat S_p}}
\newcommand{\hSpn}{{\hat S_{p_n}}}

\newcommand{\Ct}{ \mcC^+_t}
\newcommand{\Ctm}{ \mcC^+_{t_-}}
\newcommand{\hStmR}{\hat S_{t_-,R}}
\newcommand{\hStR}{\hat S_{t,R}}
\newcommand{\hSqn}{{\hat S_{q_n}}}
%\newcommand{\mcA}{\mycal A}
\newcommand{\mcZ}{\mycal Z}

\newcommand{\Cp}{ \mcC^+ }
\newcommand{\Cpe}{ \mcC^+ _\epsilon}

\newcommand{\hypo}{\,\,\mathring{\!\! \hyp}}
\newcommand{\ohypo}{\overline{\hypo}}
\newcommand{\hypot}{\,\,\mathring{\!\! \hyp_t}}
\newcommand{\hypoz}{\,\,\mathring{\!\! \hyp_0}}
\newcommand{\ohypoz}{\overline{\hypoz}}
\newcommand{\ohypot}{\overline{\hypot}}

\newcommand{\fourge}{\fourg_\epsilon}


\newcommand{\zh}{{\,\,\widetilde{\!\!\mcZ}}}
%\newcommand{\dgt}{{\mycal Z}_{\mbox{\scriptsize \rm dgt}}}

%\newcommand{\mcHp}{{\mcH^+}}
\newcommand{\mcHpz}{{\mcH^+_0}}
\newcommand{\mcHm}{{\mcH^-}}
\newcommand{\mcHmz}{{\mcH^-_0}}

\newcommand{\zN}{\mathring N}

%\newcommand{\mcY}{{\mycal Y}}
\newcommand{\mcX}{{\mycal X}}


\newcommand{\Nndg}{N_{\mbox{\scriptsize\rm  ndh}}}
\newcommand{\Ndg}{N_{\mbox{\scriptsize\rm  dh}}}
\newcommand{\Nndh}{N_{\mbox{\scriptsize\rm  ndh}}}
\newcommand{\Ndh}{N_{\mbox{\scriptsize\rm  dh}}}
\newcommand{\Naf}{N_{\mbox{\scriptsize\rm  AF}}}
\newcommand{\alpharate}{\lambda}
%\newcommand{\zalpha}{\mathring \alpha}

%\newcommand{\puncti}{a_i}
\newcommand{\ai}{\puncti}


%\newcommand{\mcS}{{\mycal S}}
\newcommand{\odocIp}{\overline{\doc}\cap I^+(\Mext)}
\newcommand{\odocup}{{\doc}\cup \mcH_0^+}
\newcommand{\llambda}{\lambda}

\newcommand{\Zd}{{\mcZ}_{\dgt}}


\newcommand{\Oma}{{}^{(a)}\Omega }
\newcommand{\Xa}{{}^{(a)}X }
\newcommand{\Sa}{{}^{(a)}S }
\newcommand{\Qea}{{}^{(a)}Q^E}
\newcommand{\Qba}{{}^{(a)}Q^B}
\newcommand{\phiea}{{}^{(a)}\Phi^E}
\newcommand{\phiba}{{}^{(a)}\Phi^B}
\newcommand{\mcHa}{{}^{(a)}\mcH}







 % The next ones are HR
\newcommand{\Sm}{\ensuremath{\Sigma_{-}}}
\newcommand{\Nt}{\ensuremath{N_{2}}}
\newcommand{\Nth}{\ensuremath{N_{3}}}



\newcommand{\jlca}[1]{\mnote{{\bf jlca:} #1}}
\newcommand{\e}{\wedge}
\renewcommand{\d}{\partial}
\newcommand{\KK}{\phi^K}
\newcommand{\Kdot}{\phi^{K}\cdot}
%\newcommand{\X.}{\phi^{X}\cdot}
\newcommand{\normK}{W}%{|K_0\e...\e K_{D-3}|^2}

\newcommand{\hyphat}{\,\,\,\widehat{\!\!\!\hyp}}
%\newcommand{\hmcM}{\,\,\,\widehat{\!\!\!\mcM}}







\newcommand{\newF}{\lambda}


%\newcommand{\Ric}{\operatorname{Ric}}
\newcommand{\Int}{\operatorname{Int}}
\newcommand{\Tr}{\operatorname{Tr}}


\newcommand{\myuu}{u}

%\newcommand{\oX}{\overline X}
%\newcommand{\oY}{\overline Y}
%\newcommand{\op}{\overline p}
%\newcommand{\oq}{\overline q}

\newcommand{\Lie}{{\mycal  L}}
\newcommand{\DD}{{\mycal  D}}
\newcommand{\PP}{{\mycal  P}}
%\newcommand{\HH}{{\mycal  H}}


\newcommand{\LL}{{\mathcal L}}


%\newcommand{\A}{{\bf A}}
\newcommand{\B}{{\bf B}}
\newcommand{\F}{{\bf F}}
%\newcommand{\I}{{\bf I}}
%\newcommand{\J}{{\bf J}}
%\newcommand{\M}{{\bf M}}
%\newcommand{\L}{{\bf L}}
%\newcommand{\O}{{\bf O}}
%\newcommand{\Q}{{\bf Q}}
%\newcommand{\R}{{\mathbb R}}
\newcommand{\U}{{\bf U}}
%\newcommand{\S}{{\bf S}}
%\newcommand{\K}{{\bf K}}
%\newcommand{\g}{{\bf g}}
%\newcommand{\t}{{\bf t}}
%\newcommand{\u}{{\bf u}}
\newcommand{\p}{{\bf p}}
\newcommand{\LLb}{{\bf \Lb}}

%\newcommand{\Ab}{\underline{A}}
\newcommand{\Eb}{\underline{E}}




%\newcommand{\nic}{}
\newcommand{\phypa}{\partial\mcS_{(a)} }
\newcommand{\Ya}{{}^{(a)}Y }
\newcommand{\Ja}{{}^{(a)}J }





%merging errors
%\newcommand{\dfrac}{\displaystyle \frac}
%\newcommand{\mod}{\ \mathrm{mod}\, } %modulo


\newcommand{\nobeijing}[1]{ \ptc{this is nobeijinged} #1}
\newcommand{\beijing}[1]{#1}


\newcommand{\lzeta}{z}

%\newcommand{\Sext}{\hyp_{\mathrm ext}}


\newcommand{\mcP}{{\mycal P}}

\newcommand{\hq}{\hat q}


\newcommand{\fourg}{{\mathfrak g }}

\newcommand{\tU}{\tilde U}


\newcommand{\twog}{h}

\newcommand{\omcN}{\,\,\,\overline{\!\!\!\mcN}}



\newcommand{\MUone}{M/\mathrm{\Uone }}%
\newcommand{\Uone}{\mathrm{U(1) }}%

\newcommand{\Mextone}{\Mext/\mathrm{\Uone }}%

%
\newcommand{\OS}{N}%
\newcommand{\tOS}{\tilde \OS}%
\newcommand{\oOS}{\mathring{\OS}}%
\newcommand{\axisym}[1]{#1}%
\newcommand{\hvphi}{{\hat\varphi}{}}%
\newcommand{\etc}{\emph{etc.}}%
\newcommand{\tGamma}{{\tilde \Gamma}}%



\newcommand{\hz}{{\hat z}{}}%

\newcommand{\ttheta}{\tilde\theta}

\newcommand{\ih}{instantaneous horizon}
\newcommand{\dih}{degenerate instantaneous horizon}
\newcommand{\nih}{nondegenerate instantaneous horizon}

\newcommand{\uS}{U_{\mathrm{Schw}}}
\newcommand{\lS}{\lambda_{\mathrm{Schw}}}
\newcommand{\alS}{\alpha_{\mathrm{Schw}}}
\newcommand{\rS}{r_{\mathrm{Schw}}}

\newcommand{\changedX}{X}
\newcommand{\Mtext}{\Mext}

\newcommand{\ii}{\mathrm{i}}
\newcommand{\Spn}{S^+_0}
\newcommand{\Spz}{S^+_0}
\newcommand{\mcEp}{{\mcE^+}}
\newcommand{\mcEpz}{{\mcE^+_0}}
\newcommand{\mcEm}{{\mcE^-}}
\newcommand{\mcEmz}{{\mcE^-_0}}


\newcommand{\jlcasug}[1]{{\color{blue}\mnote{\color{blue}{\bf jlca suggests!}
}}{\color{blue}{#1}}\color{black}\ }

\newcommand{\hfourg}{\hat \fourg}

\newcommand{\oft}{{outer future trapped}}
\newcommand{\wpt}{{weakly past trapped}}

\newcommand{\kk}[1]{}%{\mnote{{\bf If we consider the KK case:} #1}}

\newcommand{\mexp}{\mbox{\rm exp}}

\newcommand{\mzh}{\mathring h}


\newcommand{\hypwithhat}{\hathyp}
\newcommand{\hathyp}{\,\,\widehat{\!\!\hyp}}

\newcommand{\Span}{\mathrm{Span}}

\newcommand{\odoc}{\overline{\doc}}
\newcommand{\pohyp}{\partial\ohyp}



\newcommand{\opp}{\mnote{{\color{red} open problem}}}

\newcommand{\aregular}{{an {\regular}}}
\newcommand{\regular}{$I^+$--regular}%\newchange{terminology changed (macro, can be restored by resetting to ``regular")}}

\newcommand{\hthreeg}{h}


\newcommand{\zU}{\mathring U}
\newcommand{\zlambda}{\mathring \lambda}
\newcommand{\zbeta}{\mathring \beta}

\newcommand{\zalpha}{\mathring \alpha}

\newcommand{\puncti}{a_i}



\newcommand{\Cl}{{C\ell}}

\newcommand{\mcHS}{{\mcH(\hyp)}}
\newcommand{\mcHpS}{{\mcH^+(\hyp)}}
\newcommand{\mcHmS}{{\mcH^-(\hyp)}}
\newcommand{\mcH}{{\mycal H}}

\newcommand{\tY}{\widetilde{Y}}
\newcommand{\tX}{\widetilde{X}}
\newcommand{\tN}{\widetilde{N}}
\newcommand{\mycalu}{{\mycal U}}

\newcommand{\End}{{\rm \scriptsize End}}


\newcommand{\mycals}{{\mycal S}}
\newcommand{\mycalm}{{\mcM}}

\newcommand{\BA}{B_\Al}
\newcommand{\Leb}{{\mathfrak L}}

\newcommand{\Al}{{\mathcal Al}}
\newcommand{\Hausone}{\Hau^1}
\newcommand{\Htwohone}{\Hau^{2}}


\newcommand{\tA}{\theta_\Al}
\newcommand{\Hau}{{\mathfrak H}}
\newcommand{\Ar}{\mbox{\rm Area}}
\newcommand{\Arm}{\mbox{\rm Area}_{S_2}}


\newcommand{\cA}{{\mycal A}}

\newcommand{\eqs}[2]{\eq{#1}-\eq{#2}}

\newcommand{\pihyp}{\partial_\infty\hyp}
\newcommand{\cMext}{{\mcM}_{\ext}}
\newcommand{\timkd}{{\mycal T}^\flat}
\newcommand{\timku}{{\mycal T}^\sharp}


\newcommand{\cNX}{{\cal N}_X}
\newcommand{\cS}{{\cal S}}
\newcommand{\cLY}{{\mycal L}_Y}


\newcommand{\ro}{\rho}
\newcommand{\roo}{\bar{\ro}}

\newcommand{\cB}{{\mycal B}}
\newcommand{\cG}{{\mycal G}}
\newcommand{\cCak}{{\cC}^\alpha_k}


\newcommand{\wnc}{weakly null convex}

\newcommand{\bmcM}{\,\,\,\,\overline{\!\!\!\!\mycal M}}

\newcommand{\vx}{{\vec x}}
\newcommand{\sHh}{\Sigma_{\mcH}}
\newcommand{\sh}{\sHh}%{\Sigma_{\mcH}}
\newcommand{\sdh}{\Sigma_{\dot \cH}}
\newcommand{\vh}{{\vec h}}
\newcommand{\vn}{{\vec n}}
\newcommand{\vy}{{\vec y}}
\newcommand{\vz}{{\vec z}}
\newcommand{\vg}{\gamma}
\newcommand{\dG}{\dot \Gamma}
\newcommand{\tgs}{{t(s)}}
\newcommand{\pxhere}{{\phi_{\vx}(s)}}
\newcommand{\pxpm}{{\phi_{\pm}(s)}}
\newcommand{\dvg}{\dot \vg}
\newcommand{\dH}{\dot{\mcH}}
\newcommand{\Htwo}{\cH_g^2}
\newcommand{\Ltwo}{{\cal L}_{h_0}^2}
\newcommand{\Sect}[1]{Sect.~\ref{#1}}

\newcommand{\cMextw}{{\mycal M}_{\ext}^-}
\newcommand{\event}{{\mycal E}}
\newcommand{\eventw}{{\mycal E}^-}

\newcommand{\cHH}{{\mathcal H}}
\newcommand{\cF}{{\mathcal F}}


\newcommand{\AFG}{Anderson-Fefferman-Graham}

\newcommand{\hso}{hypersurface--orthogonality }

\newcommand{\hchit}{{}^t{}\hchi}
\newcommand{\hchibt}{{}^t{}\hchib}

\newcommand{\tcM}{\,\,\,\,\widetilde{\!\!\!\!\cM}}

\newcommand{\hmcM}{\,\,\,\,\widehat{\!\!\!\!\mcM}}
\newcommand{\MRRR}{\mcM_R}
\newcommand{\beq}{\begin{equation}}
\newcommand{\sgn}{\ \mbox{sgn}}
\newcommand{\massnor}{\dfrac{1}{4\omega_n}}
\newcommand{\massnortwo}{\dfrac{1}{8\omega_n}}
\newcommand{\pnorm}{\dfrac{1}{2\omega_n}}
\newcommand{\Ra}{\Rightarrow}
\newcommand{\ep}{\epsilon}
\newcommand{\vp}{\varphi}
\newcommand{\wt}{\widetilde}
\newcommand{\wh}{\widehat}

\newcommand{\ra}{\rightarrow} \newcommand{\rai}{\rightarrow\infty}
\newcommand{\rewrite}{\ptc{rewrites}}
\newcommand{\gaz}{\gamma_0}
\newcommand{\Spb}{{\frak S}}
\newcommand{\Rn}{\,{}^{n}\!R}
\newcommand{\tihyp}{\,\,\widetilde{\!\!\hyp}}%
\newcommand{\tx}{x}%

\newcommand{\cb}{\mathrm{cb}}
\newcommand{\fcb}{\mathrm{fcb}}
\newcommand{\fcbe}{future \cbe}
\newcommand{\fcbes}{future \cbes}
\newcommand{\cbe}{conformal boundary extension}
\newcommand{\cbes}{conformal boundary extensions}
\newcommand{\spa}{{\mathrm{space}}}


\newcommand{\mM}{{\mathring{M}}}

\newcommand{\hpsi}{\hat \psi}
\newcommand{\reword}{\ptc{reworded}}

\newcommand{\oX}{\overline X}
\newcommand{\oY}{\overline Y}
\newcommand{\op}{\overline p}
\newcommand{\oq}{\overline q}



\newcommand{\rd}{\,{ d}} % exterior differential



\newcommand{\mH}{{\mycal H}}%{{\mathscr H}}
\newcommand{\mHS}{{\mH}_{\Sigma}}
\newcommand{\bp}{p}%{\mathbf{p}}
\newcommand{\bd}{\mathbf{d}}
\newcommand{\bL}{\mathbf{L}}
%\newcommand{\bpi}{{\pi}\!\!\!\pi}
\newcommand{\bpi}{\pi}%{\underline{\pi}}
%\newcommand{\bpi}{{\mathscr p}}
\newcommand{\bbpi}{{\mbox{\boldmath$ \pi$}}}
%\newcommand{\bbpi}{\underline{\pi}}%{\underline{\underline{\pi}}}
%\newcommand{\bcL}{{\mathbf{\cal L}}}
\newcommand{\bcL}{{\mbox{\boldmath$ {\cal L}$}}}%
\newcommand{\caL}{{{\cal L}}}
\newcommand{\cLX}{{\lie_X}}
\newcommand{\caD}{{{\cal D}}}



\newcommand{\cutscri}{S}
\newcommand{\cPcosm}{{\mycal P}_{\mbox{\rm \scriptsize cosm}}}
\newcommand{\cMp}{M_{(\threegamma ,\threeP)}}
\newcommand{\ip}{i}



\newcommand{\tilh}{\tilde h} % metric induced by the conformal metric on S^2
 \newcommand{\DG}{D} % zbior odwzorowan konforemnych

 \newcommand{\iadsa}{\sqrt{{r^2\over\ell^2}+k }\;}
\newcommand{\adsa}{\frac{1}{\iadsa}}
\newcommand{\cPb}{{\cP}_{\text{\rm\scriptsize adS}}}
\newcommand{\Sext}{\hyp_{{\text{\scriptsize\rm ext}}}}



      \newcommand{\bh}{{\breve h}} % standard metric on S^2
 \newcommand{\taum}{{\tau_{-}}}
 \newcommand{\taumn}{-1}
 \newcommand{\phield}{{f}}
\newcommand{\phieldone}{{\varphi}}
\newcommand{\phieldtwo}{{\pi}}
 \newcommand{\tauz}{{\tau_{0}}}
      \newcommand{\TB}{Trautman--Bondi\ }


\newcommand{\hamX}{{\mathscr{X}}}
\newcommand{\jky}{{ v}}
\newcommand{\scrimap}{{\sigma}} %odwzorowanie opisujace dynamike na Scri
\newcommand{\fscri}{{\chi}} % wartosc pola skalarnego na Scri

\newcommand{\Sscr}{\Sigma_{\scrip}}
\newcommand{\iscr}{i_{\scrip}}
\newcommand{\iS}{i_{\Sigma}}
\newcommand{\iSs}{i_{\Sscr}}
\newcommand{\PhiS}{\Phi_{\Sigma}}
\newcommand{\PhiSscr}{\Phi_{\Sscr}}
\newcommand{\PhibS}{\Phi_{\bSigma}}
\newcommand{\PsiS}{\Psi_{I\times\Sigma}}
\newcommand{\psiS}{\psi_{I\times\Sigma}}
\newcommand{\PsiScr}{\Psi_{I\times\Sscr}}
\newcommand{\psiScr}{\psi_{I\times\Sscr}}

\newcommand{\frg}{{\mathfrak g}} % determinant of the metric
\newcommand{\fb}{{\mathfrak b}} % determinant of the background metric
\newcommand{\zo} {\mathring{\omega}} % koneksja metryki tla
\newcommand{\hzo} {\widehat{\zo}{}} % koneksja metryki tla
\newcommand{\oeps}{o(r^{-2\alpha})}
\newcommand{\oepsb}{o(r^{\beta-2\alpha})}
\newcommand{\myvareps}{}
\newcommand{\newa}{c}
\newcommand{\T}{\Bbb T}

\newcommand{\tH}{{H}}
\newcommand{\tV}{\tilde{V}}


\newcommand{\sRz} {\mathring{\sigma}_R} % odleglosc geodezyjna metryki tla
\newcommand{\sR} {\sigma_R} % odleglosc geodezyjna metryki
\newcommand{\zn} {\mathring{\nabla}} % pochodna metryki tla
\newcommand{\twoM}{\breve{M}}
\newcommand{\fzero}{n}
\newcommand{\A}{A} \newcommand{\ta}{a} \newcommand{\ha}{a}
%\newcommand{\hb}{b}
\newcommand{\hc}{c} \newcommand{\gf}{f} \newcommand{\ce}{\beta}
\newcommand{\hv}{{\hat v}}
\newcommand{\he}{{\hat e}}


\newcommand{\hypext}{{\hyp_{\ext}}}


\newcommand{\fg}{{}^4{g}}
\newcommand{\ac}{\zeta}
\newcommand{\cM}{\mycal M} % space-time
\newcommand{\localcM}{M} % space-time
\newcommand{\mn} {\twoM} %{{}^{n-1}M} %the n-1 dimensional manifold
\newcommand{\zRs} {\mathring{R}} % Ricci itd tla
\newcommand{\zRm} {\mathring{R}} % Ricci itd tla

\newcommand{\gp}{g}


\newcommand{\otg}{\mathring{\!\threegamma }\,}
\newcommand{\cpp}{\psi_{(\threegamma ,\threeP)}}
\newcommand{\cop}{{\cal O}_{(\threegamma ,\threeP)}}
\newcommand{\Sint}{\Sigma_{\inter}}
\newcommand{\Siext}{\Sigma_{\ext}}
\newcommand{\inter}{{\mbox{\rm\scriptsize int}}}
%\newcommand{\ext}{{\mbox{\rm \scriptsize ext}}}
\newcommand{\cPadm}{{\mycal P}_{\mbox{\rm \scriptsize ADM}}}
\newcommand{\htg}{\widehat{\threegamma }}
\newcommand{\htgh}{\widehat{\threegamma h}}
\newcommand{\rK}{\mathring{K}}
\newcommand{\rP}{\mathring{\threeP}}
\newcommand{\rPh}{\mathring{\threePh}}
\newcommand{\cPk}{{\mycal P}_{\rP}}
    \newcommand{\threegammah}{\threegamma _{ij}}
    \newcommand{\threePh}{\threeP^{kl}}


\newcommand{\arcsh}{{\rm argsh}}

                               %to the model space
\newcommand{\lapse}{{\nu}} % the lapse function on the model space
\newcommand{\shift}{{\beta}} % the shift vector field on the model
                             % space
\newcommand{\threeP}{{\pi}} %three dimensional ADM momentum pulled back
                               %to the model space
\newcommand{\tildeg}{{\tilde g}} % conformally rescaled metric
\newcommand{\hst}{{\breve{h}}} % standard round metric on the two
                              % sphere

%\newcommand{\Freud}{{\scriptsize\mbox{Freud}}}
\newcommand{\Freud}{{\mbox{\scriptsize boundary}}}
\newcommand{\HF}{H_{\Freud}}
\newcommand{\HFren}{H_{\Freud}^{\ren}}
\newcommand{\hype}{{\hyp^{\epsilon}}}


\newcommand{\pblurb}{(X,{\partial\hyp})}
\newcommand{\blurb}{(X,{\hyp})} % {(X,{\hyp},\Jped)}
\newcommand{\blurbe}{(X,{\hype})} %{(X,{\hype},\Jped)}
\newcommand{\HFh}{H_{\Freud}\blurb}
\newcommand{\HFhe}{H_{\Freud}\blurbe}
\newcommand{\Hh}{H\blurb}
\newcommand{\Hhe}{H\blurbe}


\newcommand{\bA}{\,\,{\stackrel{\circ}{\!\!A}}\vphantom{A}}

\newcommand{\FS}       %{F_1} %
                  {F}
                       %{F_{\mbox{\scriptsize volume}}}

\newcommand{\HS} %{F_2}
       {H_{\mbox{\scriptsize volume}}}

\newcommand{\ren}{\mbox{\scriptsize normalised}}


\newcommand{\cgg}{c}
\newcommand{\cgamma}{c}

\newcommand{\hb}{\HH}
\newcommand{\QED}{\qed}


\newcommand{\Norm}[2]{\Vert#1\Vert_{#2}}

\newcommand{\half}{\frac 12}

\newcommand{\zei}{{\mathring{e}_i}}
\newcommand{\zej}{{\mathring{e}_j}}

\newcommand{\tauLambda}{\frac{n-2}{4n}\tau^2_\Lambda}
\newcommand{\JDG}{Jour.~Diff.~Geom.}
\newcommand{\CPAM}{Commun. Pure Appl.\ Math.}
\newenvironment{ober}%
{\ptc{this should be removed in the oberwolfach version}}%


\newcommand{\tGam}{{\widetilde \Gamma}}
\newcommand{\tD}{{\widetilde D}}
\newcommand{\tL}{{\widetilde L}}
\newcommand{\tR}{{\widetilde R}}

\newcommand{\trh}{\mathrm{tr}_h}


\newcommand{\tnab}{\tilde \nabla}
\newcommand{\dotJ}{{\dot J}}
\newcommand{\Remarkn}[1]{{\bf Remark #1:}}
\newcommand{\zthe}{\mathring{\theta}}
\newcommand{\zD}{\mathring{D}}%
\newcommand{\zA}{\mathring{A}}%
\newcommand{\zE}{\mathring{E}}%
\newcommand{\zB}{\mathring{B}}%
\newcommand{\ze}{\mathring{e}}%
\newcommand{\zK}{\mathring{K}}%
\newcommand{\zomega}{\mathring{\omega}}%
\newcommand{\cosm}{\alpha}%
\newcommand{\I}{\sqrt{-1}}%
\newcommand{\cosmi}{\frac{\cosm \I}{2}}%
\newcommand{\cK}{{\cal K}}%
\newcommand{\mcA}{{\mycal A}}%
\newcommand{\mcT}{{\mycal T}}%
\newcommand{\mcE}{{\mycal E}}%

\newcommand{\HHKm}{{\mathbb{H}_{\cK_-}}}%


\newcommand{\ihyp}{\,\,\mathring{\!\!\hyp}}
\newcommand{\ourU}{\mathbb U}%
\newcommand{\eeal}[1]{\label{#1}\end{eqnarray}}
\newcommand{\id}{\textrm{id}}%\newcommand{\id}{\textrm{id}}%
\newcommand{\C}{{\mathbb C}}%\newcommand{\C}{\mathbb C}%
%\newcommand{\ga}{{\gamma}}
\newcommand{\bed}{\begin{deqarr}}
\newcommand{\eed}{\end{deqarr}}
\newcommand{\bedl}[1]{\begin{deqarr}\label{#1}}
\newcommand{\eedl}[2]{\arrlabel{#1}\label{#2}\end{deqarr}}

\newcommand{\loc}{\textrm{\scriptsize\upshape loc}}
\newcommand{\zmcH}{\mathring{\mycal H}}
\newcommand{\tg}{{\widetilde{g}}}
\newcommand{\can}{g_{\cerc^{n-1}}}%{\mathrm{can}}
\newcommand{\checked}{\ptc{checked}}
\newcommand{\mzD}{D}
\newcommand{\pM}{\partial M }
\newcommand{\pN}{\partial N}

\newcommand{\dga}{\sigma_{g_a}}
\newcommand{\dgo}{\sigma_{g_1}}
\newcommand{\dgt}{\sigma_{g_2}}
\newcommand{\phot}{\phi_{12}}
\newcommand{\phto}{\phi_{21}}
\newcommand{\doto}[1]{\frac{d #1}{d s}}
\newcommand{\mcO}{{\mycal O}}
\newcommand{\mcU}{{\mycal U}}


\newcommand{\new}{\ptc{new addition, needs proofreading}}
\newcommand{\newsec}{\ptc{new section, needs proofreading}}
%\newcommand{\mcM}{{\mycal M}}
\newcommand{\mcN}{{\mycal N}}
\newcommand{\mcK}{{\mycal K}}

%\newcommand{\loc}{{\textrm{loc}}}
\newcommand{\bel}[1]{\begin{equation}\label{#1}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\bean}{\begin{eqnarray}\nonumber}
%\newcommand{\eea}{\end{eqnarray}}
%\newcommand{\nn}{\nonumber}
\newcommand{\beal}[1]{\begin{eqnarray}\label{#1}}
\newcommand{\eea}{\end{eqnarray}}

\newcommand{\distb}{\dist_{\backmg}}
\newcommand{\dist}{\mathrm{dist}}
\newcommand{\lorentz}{\sigma}
\newcommand{\lorp}{\lorentz_p} % world function
\newcommand{\nn}{\nonumber}
\newcommand{\Eq}[1]{Equation~\eq{#1}}
\newcommand{\Eqsone}[1]{Equations~\eq{#1}}
\newcommand{\Eqs}[2]{Equations~\eq{#1}-\eq{#2}}
\def\INCLUDE#1{\typeout{:<+ #1.tex}\include{#1}\typeout{:<-}}
\newcommand{\qed}{\hfill $\Box$ \medskip}
\newcommand{\proof}{\noindent {\sc Proof:\ }}
%\newcommand{\remark}{\noindent {\bf Remark:\ }}
\newcommand{\be}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\eeqa}{\end{eqnarray}}
\newcommand{\beqan}{\begin{eqnarray*}}
\newcommand{\eeqan}{\end{eqnarray*}}
\newcommand{\ba}{\begin{array}}
\newcommand{\ea}{\end{array}}

\newcommand{\cC}{{\cal C}}
\newcommand{\backmg}{h} %background Riemannian metric
\newcommand{\Id}{\mbox{\rm Id}} %identity matrix
\newcommand{\const}{\mbox{\rm const}} %constants

\newcommand{\hyp}{\mycal S}
\newcommand{\HH}{{\cal H}}
\newcommand{\Hk}[1]{{\cal H}_k^{#1}}
\newcommand{\Hak}{{\cal H}_{k} ^{\alpha}}
\newcommand{\sigxx}[1]{\Sigma_{x_2,x_1,#1}}
\newcommand{\sigx}[1]{\Sigma_{x_1,#1}}
\newcommand{\demi}{{1\over 2}}
\newcommand{\emoins}{E_{-}^{\mu}}
\newcommand{\eplus}{E_{+}^\mu}
\newcommand{\nmu}{\nabla_\mu}
\newcommand{\pmu}{\partial_\mu}
\newcommand{\px}{\partial_x}
\newcommand{\db}{D^\beta}
\newcommand{\pb}{\partial^\beta}
\newcommand{\xadu}{x^{-2\alpha-1+2\beta_1}}
%\newcommand{\mycal}{\cal}
\newcommand{\mcM}{{\mycal M}}
\newcommand{\mcD}{{\mycal D}}
\newcommand{\dirac}{\mathrm{Dirac}}
%Lee \newcommand{\dirac}{\mcD}
\newcommand{\bdirac}{\,\,\overline{\!\!\dirac}}%{\mathrm{Dirac}}
%\newcommand{\mcU}{{\mycal U}}
\newcommand{\mcW}{{\mycal W}}
\newcommand{\mcV}{{\mycal V}}
\newcommand{\cO}{{\cal O}}
\newcommand{\cU}{{\cal U}}
\newcommand{\cW}{{\cal W}}
\newcommand{\cV}{{\cal V}}
\newcommand{\spacetime}{({\mycal M} , g)}
\newcommand{\unphyspace}{{ \tilde {\mycal M}}}
\newcommand{\err}{\zeta} % error function, determines how fast things go to zero
\newcommand{\prho}{p}
\newcommand{\dx}{\,dx}
\newcommand{\Img}{\mbox{Im}\,}
\newcommand{\mcY}{{\mycal Y}}

\newcommand{\scri}{{\mycal I}}%
\newcommand{\scrip}{\scri^{+}}%
\newcommand{\scrim}{\scri^{-}}%
\newcommand{\scripm}{\scri^{\pm}}%
\newcommand{\scrp}{{\mycal I}^{+}}%
\newcommand{\Scri}{\scri}
%\renewcommand{\cal}{\mycal}

\newcommand{\novec}[1]{{#1}}
%\newcommand{\bysame}{---}
%\newcommand{\proof}{{\sc Proof:}\ }
\newcommand{\proofend}{\hfill\ $\Box$}
%\renewcommand{\themnotecount}{\thesection.\arabic{mnotecount}}

\newcommand{\mnote}[1]%{}
{\protect{\stepcounter{mnotecount}}$^{\mbox{\footnotesize
$%\!\!\!\!\!\!\,
\bullet$\themnotecount}}$ \marginpar{%\color{red}%
\raggedright\tiny\em
$\!\!\!\!\!\!\,\bullet$\themnotecount: #1} }

\newcommand{\warn}[1]%{}%{}
{\protect{\stepcounter{mnotecount}}$^{\mbox{\footnotesize
$%\!\!\!\!\!\!\,
\bullet$\themnotecount}}$ \marginpar{%\color{red}%
\raggedright\tiny\em
$\!\!\!\!\!\!\,\bullet$\themnotecount: {\bf Warning:} #1} }

%\newcommand{\mnote}[1]{}

\newcommand{\zvarphi}{{\mathring{\varphi}}}

\newcommand{\Omnote}[1]{\mnote{{\bf OL:} #1}}
\newcommand{\Pmnote}[1]{{\bf PTC:} #1}
\newcommand{\R}{\mathbb R}
\newcommand{\Hilb}{\HH}
\newcommand{\N}{\mathbb N}
\newcommand{\Z}{\mathbb Z}
\newcommand{\Q}{\mathbb Q}
\newcommand{\bM}{\overline{\! M}}
\newcommand{\tp}{\tilde{\! \partial}}
\newcommand{\backg}{b}
%\newcommand{\pM}{\partial M}
\newcommand{\eq}[1]{(\ref{#1})}
\newcommand{\ga}{{\gamma}}
\newcommand{\Mext}{M_\ext}
\newcommand{\ext}{\mathrm{ext}}
\newcommand{\mfd}{\nabla\hskip -0.45truecm \not\hskip 0.45truecm}
\newcommand{\mtd}{D\hskip -0.25truecm / \,}
\newcommand{\trg}{{\mathrm{tr}_g}}
\newcommand{\divE}{\mathrm{div}(E)}
\newcommand{\divB}{\mathrm{div}(B)}

\newcommand{\rspone}{\rangle_{\!{}_{1}}}
\newcommand{\rsptwo}{\rangle_{\!{}_{2}}}

\newcommand{\dea}{{\cal D}_{e_{A}}}
%\newcommand{\loc}{\mbox{{\rm\scriptsize loc}}}
\newcommand{\xa}{x^ \alpha}
\newcommand{\coa}{\cC _0 ^\alpha}
\newcommand{\boa}{{\cal B} _0 ^\alpha}
\newcommand{\cob}{\cC _0 ^\beta}
\newcommand{\Hbk}{\Hk \beta}
\newcommand{\GG}{{\cal G}}
\newcommand{\Gk}[1]{\GG_k ^{#1}}
\newcommand{\Gak}{\Gk \alpha}
\newcommand{\gok}{\Gk 0}
\newcommand{\Gbk}{\Gk \beta}
\newcommand{\tM}{\;\;\;\widetilde{\!\!\!\!\!\cal M}}
\newcommand{\hmcK}{\;\;\;\widehat{\!\!\!{\mcK}}}
\newcommand{\dmu}{d\mu} %measure on M
\newcommand{\volu}{\,d \nu} %measure on the boundary of M
\newcommand{\dnu}{\volu} %measure on the boundary of M

\newcommand{\ooi}{\Omega_i} % product coordinate neighborhoods near
                            % the boundary
\newcommand{\volume}{\,d^{n}\mu}
\newcommand{\ptc}[1]{\mnote{{\bf ptc:}#1}}
\newcommand{\agp}[1]{\mnote{{\bf agp:}#1}}
\newcommand{\jc}[1]{\mnote{{\bf jc:}#1}}

\newcommand{\Hess}{\mathrm{Hess}\,}
\newcommand{\Vect}{\mathrm{Vect}}
\newcommand{\complementaire}{\complement}

\newcommand{\mcDpmS}{{\mycal D}^\pm(\hyp)}

\newcommand{\diag}{\mbox{\rm diag}}
\newcommand{\Lg}{{g}} % four dimensional Lorentzian metric
\newcommand{\LM }{{ \mcM }} % spacetime
\newcommand{\up }{{}^{\sharp}} % this takes indices up
\newcommand{\down}{{}_{\flat}} % this takes indices  down
\newcommand{\Ric}{\mbox{\rm Ric}}
\newcommand{\Riem}{\mbox{\rm Riem}}

\newcommand{\mcC}{{\mycal C}}
\newcommand{\mcS}{{\mycal S}}
\newcommand{\mcL}{{\mycal L}}
\newcommand{\mcR}{{\mycal R}}

\newcommand{\beqar}{\begin{deqarr}}
\newcommand{\eeqar}{\end{deqarr}}

\newcommand{\beaa}{\begin{eqnarray*}}
\newcommand{\eeaa}{\end{eqnarray*}}

\newcommand{\tr}{\mbox{tr}}
\newcommand{\zg}{\mathring{g}}
\newcommand{\zG}{\mathring{\Gamma}}
\newcommand{\zGamma}{\mathring{\Gamma}}
\newcommand{\znabla}{\mathring{\nabla}}
\newcommand{\zR}{\mathring{R}}

\newcommand{\hamiltonian}{Hamiltonian } %decide lower or upper case?
\newcommand{\Lagrangian}{Lagrangian } %decide lower or upper case?
\newcommand{\Bgamma}{{B}} % koneksja tla
\newcommand{\bmetric}{{b}} % metryka tla

\newcommand{\Kp}{{\frak g}} %{\pi}} % kontrawariantna gestosc metryki
                            %na czasoprzestrzeni
\newcommand{\KA}{p} % ped sprzezony do kontrawariantnej gestosci
                    % metryki (A duze w innych pracach JK i JJ)
\newcommand{\jexp}[1]{{\rm e}^{#1}}
%\newcommand{\kolo}[1]{\stackrel{\circ}{#1}}
\newcommand{\ve}{\varepsilon}
\newcommand{\gthreeup}{\,{}^3g} %three dimensional metric in
                                %space--time, used for the inverse

\newcommand{\bfJ}{{\mathbb J}}

\newcommand{\varomega}{\omega} % conformal factor on a fixed hypersurface
\newcommand{\hvaromega}{\hat{\varomega}} % conformal factor on a fixed hypersurface,
                                    % extended beyond the boundary
\newcommand{\hdotvaromega}{\widehat{\dot{\varomega}}} % conformal factor on a fixed hypersurface,
                                    % extended beyond the boundary
\newcommand{\toto}{\R}% \toto used to be \R^*_+, replaced by \R
\newcommand{\tLambda}{\tilde\Lambda} % tensor densities
\newcommand{\newH}{\widehat H}


\newcommand{\conffour}{\varOmega} % four dimensional conformal factor
                                  % here
\newcommand{\confthree}{\varomega} % three dimensional conformal factor
                                  % here
\newcommand{\dconfthree}{\dvaromega} % time derivative of the three
                                     % dimensional conformal factor
\newcommand{\extL}{L} % trace free part of the extrinsic curvature of
                      % a three dimensional hypersurface
\newcommand{\textL}{\tilde L} % conformally rescaled trace free part
                              % of the extrinsic curvature of
                      % a three dimensional hypersurface
\newcommand{\textK}{\tilde K} % conformally rescaled extrinsic curvature of
                      % a three dimensional hypersurface
\newcommand{\tK}{\tilde K} % trace of the conformally rescaled
                           % extrinsic curvature of
                      % a three dimensional hypersurface
\newcommand{\tlambda}{\tilde \lambda} % extrinsic curvature of
                      % a two  dimensional boundary in a conformal picture
\newcommand{\ccalD}{\;\breve{\!\cal D}}


\newcommand{\lie}{{\pounds}} %Lie derivative
%\newcommand{\lie}{{\cal L}}
%\def\varOmega{{\it\Omega}}
%\newcommand{\varOmega}{{\mathit{\Omega}}}
%\def\varOmega{{\Omega}}
\newcommand{\rdphi}{\rd \varphi}
\newcommand{\rdS}{\rd S} % formy objetosciowe trzeba zmienic na dS



\newcommand{\Gtwo}{\two\Gamma}
\newcommand{\Gst}{\breve\Gamma}

\newcommand{\ourW}{\mathbb W}

\newcommand{\dvaromega}{\dot\varomega} %time derivative of the conformal factor
\newcommand{\ohyp}{\,\,\overline{\!\!\hyp}} % closure of the initial data hypersurface
\newcommand{\thyp}{\tilde\hyp}
\newcommand{\hhyp}{\,\,\widehat{\!\!\hyp}\,} % extension of the initial data
                               % hypersurface beyond Scri
\newcommand{\tmet}{\tilde\met} % conformally rescaled metric on a
                               % three dimensional manifold
\newcommand{\hmet}{\hat\met}
\newcommand{\met}{\gamma} % metric induced on a three dimensional hypersurface
\newcommand{\extK}{K} % extrinsic curvature of a three dimensional hypersurface
\newcommand{\tiext}{\tilde\extK } % conformally rescaled extrinsic


\newcommand{\Jphi}{f}%{{\tilde f}}%{\phi} % pole skalarne fizyczne
\newcommand{\dotphi}{\dot\phi}
\newcommand{\dotJphi}{\dot\Kphi}
\newcommand{\dotpi}{\dot\pi}
\newcommand{\dotJpi}{\dot\Jpi}
\newcommand{\Jpsi}{\tilde f}%{\psi} % pole skalarne niefizyczne
\newcommand{\Jpi}{{\tilde p}}%{\pi} %ped konforemnie przetransformowany
\newcommand{\Jped}{p}%{\pi} % ped na przestrzeni fizycznej
\newcommand{\tphi}{{\tilde\phi}}
\newcommand{\tpi}{{\tilde\pi}}
\newcommand{\aalpha}{\lambda} % funkcja wyznaczajaca supertranslacje
\newcommand{\przecinekJped}{}
\newcommand{\bF}{{\widetilde F}}
%\newcommand{\bi}{i_{\bSigma}}%{{\tilde \imath}}
\newcommand{\bhyp}{{\widetilde \hyp}}
\newcommand{\bSigma}{{\widetilde \Sigma}}
\newcommand{\cP}{{\cal P}}
%\newcommand{\cDX}{{\cal D}_X}
\newcommand{\cDX}{{\mathscr D}_X}
\newcommand{\dg}{\ \!\!\vartriangle\!\!\Kp}%{\Delta\Kp}{\blacktriangle\Kp}%
                                         %roznica metryki a metryka tla


%\newcommand{~\cite}[1]{~\cite{#1}}

\newcommand{\refcite}[1]{\cite{#1}}
\newcommand{\bhindex}[1]{\index{#1}}

\newcommand{\xflat}{X^\flat}
\newcommand{\kflat}{K^\flat}
\newcommand{\yflat}{Y^\flat}
\newcommand{\OOmega}{\omega}
\newcommand{\ptcKcite}[1]{.\cite{#1}}

\newcommand{\cimkd}{{\mycal C}^\flat}
\newcommand{\cimku}{{\mycal C}^\sharp}
\newcommand{\proj}{\textrm{pr}}
\newcommand{\Mclosed}{\bcM}%{\hskip10pt {\overline{\phantom{I}}\hskip-15pt{\mycal M}}}
\newcommand{\cg}{\,{\tilde {\!g}}}

\newcommand{\bcM}{{\,\,\,\overline{\!\!\!\mcM}}}%{\,\,\,\,\widetilde{\!\!\!\!\cM}}
%\newcommand{\tcM}{\,\,\,\,\widetilde{\!\!\!\!\cM}}
\newcommand{\hJ}{{\hat J}}
\newcommand{\sthd}{{}^{\star_g}}
\newcommand{\hG}{\widehat \Gamma}
\newcommand{\hD}{\widehat D}
\newcommand{\hxi}{\hat \xi}
\newcommand{\hxib}{\hat{\xib}}
\newcommand{\heta}{\hat \eta}
\newcommand{\hetab}{\hat{\etab}}
\newcommand{\home}{\hat{\omega}}
\newcommand{\mcB}{{\mycal B}}
\newcommand{\homb}{\hat{\underline\omega}}
\newcommand{\doc}{\langle\langle \mcM\rangle\rangle}
%\newcommand{\Sext}{\hyp_{\mathrm ext}}

\newcommand{\hg}{{\hat g}}
\newcommand{\mcEh}{{{\mycal E}^+_\hyp}}

%\newcommand{\cM}{\mycal M}
\newcommand{\cN}{\mycal N}
\newcommand{\cE}{\mycal E}
\newcommand{\gcirc}{{\mathring{g}}_{ab}}
\let\a=\alpha\let\b=\beta \let\g=\gamma \let\d=\delta\let\lb=\lambda
\newcommand{\sts}{space-times}
\newcommand{\calM}{{\mcM}}
\newcommand{\calH}{{\mcH}}
\newcommand{\el}{e^{2\lb}}
\newcommand{\hysf}{hypersurface}
%\newcommand{\mcH}{{\cal H}}


\newcommand{\hS}{\hat{\Sigma}}
\newcommand{\hX}{\hat{X}}
\newcommand{\pS}{\partial\Sigma}
\newcommand{\ps}{\pS}
\newcommand{\dS}{\dot{\Sigma}}
\newcommand{\pdS}{\partial\dS}
\newcommand{\pds}{\pdS}
\newcommand{\pd}{\partial_{\doc}}
\newcommand{\ddoc}{\dot{\doc}}
\newcommand{\hp}{\hat{\pi}}
\newcommand{\bcU}{\breve{\cal U}}
%\newcommand{\cU}{{\cal U}}
%\newcommand{\mcN}{{\cal N}}
%\newcommand{\cO}{{\cal O}}
\newcommand{\mcNX}{{\cal N}_X}
\newcommand{\calS}{{\cal S}}
%\newcommand{\cV}{{\cal V}}
%\newcommand{\R}{\Bbb R}
%\newcommand{\ext}{{\mathrm{ext}}}
%%\newcommand{\ext}{{\scriptsize\textrm{ext}}}
%\newcommand{\Sext}{\Sigma_\ext}
\newcommand{\Snd}{\partial_{nd}\Sigma}
%\newcommand{\hg}{\hat \gamma}
%\newcommand{\tg}{\tilde \gamma}
\newcommand{\tk}{\tilde \kappa}
\newcommand{\hI}{\hat I}
%
\newcommand{\communication}{{communications}}
\newcommand{\communications}{{communications}}
\newcommand{\Proof}{\proof}
%%\newcommand{\doc}{\leftineq\rh\rightineq}
\newcommand{\ks}{{\cal K}(\Sigma)}
%\newcommand{\khs}{{\cal K}(\hS)}
\newcommand{\kds}{{\cal K}(\dS)}
\newcommand{\pkds}{\partial{\cal K}(\dS)}
%\newcommand{\Mext}{M_{\mathrm{ext}}}
%%\newcommand{\doc}{\langle \langle \Mext \rangle \rangle}
%\newcommand{\doc}{{\cal D}_{oc}}
%%\newcommand{\doc}{{\cal D}_{\cal OC}}
%%\newcommand{\doc}{{\cal D}_{oc}(\Mext)}
\newcommand{\pdoc}{\partial\doc}

\newcommand{\cf}{{\emph{ cf.}}}

\newcommand{\trho}{{\tilde \rho}}
\newcommand{\trr}{{\tilde r}}
\newcommand{\ty}{{\tilde y}}
%\newcommand{\tx}{{\tilde x}}
\newcommand{\hrho}{\hat\rho}
\newcommand{\hr}{{\hat r}}
\newcommand{\hx}{{\hat x}}
\newcommand{\hy}{{\hat y}}
\newcommand{\hvarphi}{\hat\varphi}
\newcommand{\tvarphi}{\tilde\varphi}
\newcommand{\sign}{\mathrm{sign}}

\newcommand{\gad}[1]{\gamma_{#1}}
\newcommand{\gau}[1]{\gamma^{#1}}

\newcommand{\K}{{\mathbb K}}

\newcommand{\supp}{{\mbox{\rm supp}\,}}

\newcommand{\eg}{{\emph{e.g.,\/}}}

\newcommand{\levoca}[1]{\ptc{#1}}
\newcommand{\chindex}[1]{\index{#1}}

